Sentiment Analysis Based on RoBERTa for Amazon Review: An Empirical Study on Decision Making

In this study, we leverage state-of-the-art Natural Language Processing (NLP) techniques to perform sentiment analysis on Amazon product reviews. By employing transformer-based models, RoBERTa, we analyze a vast dataset to derive sentiment scores that accurately reflect the emotional tones of the reviews. We provide an in-depth explanation of the underlying principles of these models and evaluate their performance in generating sentiment scores. Further, we conduct comprehensive data analysis and visualization to identify patterns and trends in sentiment scores, examining their alignment with behavioral economics principles such as electronic word of mouth (eWOM), consumer emotional reactions, and the confirmation bias. Our findings demonstrate the efficacy of advanced NLP models in sentiment analysis and offer valuable insights into consumer behavior, with implications for strategic decision-making and marketing practices.

==> Thesis_Title_1_/tex/glossary.tex <==
% Glossary entry definitions and acronyms
\longnewglossaryentry{sampleGlossaryEntry}{
    name={Glossary Entry},
    text={glossary entry}
}{%
This is a sample glossary entry.

Glossary entry descriptions can span multiple paragraphs.

Remember that glossaries are optional.
The glossary implementation in this template is intended to be simple, and makes use of only one package, \href{https://www.ctan.org/pkg/glossaries}{\texttt{glossaries}}. There are more flexible, and fully-featured methods for creating glossaries than the one used here.
}

\newacronym[description={A sample acroynm description}]{asa}{ASA}{A Sample Acronym}
